SPIN: Structure-Preserving Inner Offset Network for Scene Text Recognition

Arbitrary text appearance poses a great challenge in scene text recognition tasks. Existing works mostly handle with the problem in consideration of the shape distortion, including perspective distortions, line curvature or other style variations. Therefore, methods based on spatial transformers are extensively studied. However, chromatic difficulties in complex scenes have not been paid much attention on. In this work, we introduce a new learnable geometric-unrelated module, the Structure-Preserving Inner Offset Network (SPIN), which allows the color manipulation of source data within the network. This differentiable module can be inserted before any recognition architecture to ease the downstream tasks, giving neural networks the ability to actively transform input intensity rather than the existing spatial rectification. It can also serve as a complementary module to known spatial transformations and work in both independent and collaborative ways with them. Extensive experiments show that the use of SPIN results in a significant improvement on multiple text recognition benchmarks compared to the state-of-the-arts.

==> sections/1_intro.tex <==
\vspace{-0.3cm}
\section{Introduction}
Optical Character Recognition (OCR) has long been an important task in many practical applications. Recently, recognizing text in natural scene images, referred to as Scene Text Recognition (STR), has attracted great attentions due to the diverse text appearances and the extreme conditions in which these scenes are captured. Modern techniques in deep neural networks have been widely introduced \cite{CRNN,RARE,R2AM,ASTER,GRCNN,FAN,AON,SSFL,SSDAN,SRN}. %For example, Shi \etal \cite{CRNN} proposed CRNN to exploit the contexture information by combining convolutional neural networks (CNNs) and recurrent neural networks (RNNs). Lee \etal \cite{R2AM} introduced attention modeling to focus on the most reliable regions at every recurrent step. Hybrid attention methods combining various revisions have achieved great success \cite{FAN,ASTER}.

Since existing methods are quite powerful for regular text tasks, irregular shape has become a challenging yet hot interest for researchers. As spatial transformer network (STN) \cite{STN} was proposed, RARE \cite{RARE} integrated it into a mainstreaming preprocessing procedure in the STR framework before the regular encoder-decoder recognition stage. Notice that the \textit{rectification module} does not require any extra annotations yet is effective in an end-to-end network. Therefore, it was soon popularly utilized and further explored in later works \cite{AFDM,wrong,ASTER,ESIR,MORAN,ScRN}. %For example, recently, Zhan \etal \cite{ESIR} proposed line-fitting transformation to iteratively estimate the pose of text lines in scenes. Yang \etal \cite{ScRN} improved the control point prediction in STN. Luo \etal \cite{MORAN} directly predicted the location offsets of the coordinates to rectify multi-object.
\begin{figure}[!t]
	\centering
	\includegraphics[scale=0.45]{figure/intro-v3.jpg}
	\vspace{-0.7cm}
	\caption{Examples of regular and irregular scene text, where the problems of irregular case can be categorized into geometric distortion and chromatic distortion.}
	\label{fig:0}
\vspace{-0.5cm}
\end{figure}
Although almost all the existing transformations are limited to geometric rectification, shape distortions do not account for all difficult cases. Severe conditions resulting from intensity variations, poor brightness, shadow, background and imaging noise, even some insensible to human beings also contribute to hard samples for deep networks. %occlusion, low resolution,
In particular, corresponding to geometric distortion, we term these irregularities as \textit{chromatic distortions}, which are very common and intractable but attracted rare attention in STR.
%, which are exceedingly common and intractable in real world. }
%Existing rectification networks \cite{RARE,ESIR,MORAN,ScRN} were motivated to recognize images as shown in Fig. \ref{fig:0}(b), but samples such as Fig. \ref{fig:0}(c) and (d) were left intractable. Until now, chromatic problems have attracted rare attention in scene text recognition tasks.
{%\color{red}
%Version1: Landau \etal \cite{landau1988importance} stated that humans prefer to categorize objects based mainly on their shapes (only supplemented by colors and brightness information), while networks are sensitive to color deviation. Similar structure patterns while changing perceptible deviation on colors lead to fatal damage to network recognition results, which may not hurt human classifiers. Therefore, we intuitively intend to design a novel rectification module for adaptively reducing the burdens of visual inference through adjusting the distributions of image color. It transforms the images to chromatic styles which is most suitable for the downstreaming recognition task through end-to-end training.
%Version0: As work \cite{landau1988importance} stated that humans prefer to categorize objects based on their shapes rather than colors, even the geometric distorted texts in Fig. \ref{fig:0}(b) can be easily recognized by humans on condition that \textit{the shapes of objects are clear enough}. Therefore, we intuitively intend to design a novel network for preserving the important shapes of texts and reducing the burdens of visual inference through adjusting the distributions of image color.
Early work \cite{landau1988importance} stated that humans prefer to categorize objects based on their shapes, even the geometric distorted texts in Fig. \ref{fig:0}(b) can be easily recognized on condition that \textit{the shapes of objects are well preserved}.
%While shape is not clear enough caused by chromatic distortion like (c) and (d), recognition becomes much harder.
However, chromatic distortion leads to unclear shapes like in Fig.\ref{fig:0}(c) and (d), thus, recognition becomes much harder.
To reduce burdens of STR, we are inspired to rectify the chromatic distortion to restore shapes of texts.
%So we are inspired to design a network for preserving the important shapes of texts.
That is, to design intensity manipulations towards variable distorted conditions.
}

%Recent works \cite{hosseini2018semantic,SPT} focused on the revelation of the model's vulnerability to intensity-related noises. In detail, all the pixels with the same intensity are denoted as a \textit{structure-pattern} (short in \textit{pattern} below).
%Observing intrinsic features learned from networks are sensitive to color deviation, \cite{SPT} misled the models through transforming the intensity level of \textit{pattern}s.
%Contrary to their usage, we are motivated to apply intensity manipulation for alleviating chromatic distortions.

%It transforms the images to chromatic styles which is most suitable for the downstreaming recognition task through end-to-end training
%we try to apply intensity manipulations to alleviate the chromatic outliers,
%opposite to the former usage of destroying deep learning visual tasks.
%The difficulty of rectifying chromatic distortions lies in that the chromatic outliers not only contain inconsistent intensities with the normal patterns, but also consistent intensities, which cannot be directly separated and lead to visual inference.
%However, \textit{rectifying is always harder than destroying}.
Usually, chromatic distortions can be grouped into two cases (in Fig. 2) named \textit{inter-pattern} and \textit{intra-pattern} problems (explained later).
Here we denote all the pixels with the same intensity as a \textit{structure-pattern} (short in \textit{pattern}). 
%Therefore, pixels with the same intensity-level in an image are regarded as a single \textit{pattern}.
Assuming an ideal condition that the images to be identified are clearly composed of two distinct \textit{pattern}s: the intended text \textit{pattern} and the uncaring background \textit{pattern}, networks can focus on the intrinsic shape or features of the text \textit{pattern}.
However, real scenes are far more complex than the above assumption,
ubiquitous images can meet diverse chromatic challenges. 
%which can be grouped into 2 cases (as Fig.2):
{%\color{blue}
In detail of two chromatic distortion types, 
(a) \textit{inter-pattern problem} means noise \textit{pattern}s are close to the text \textit{pattern}s (\eg poor contrast or brightness) or intensities of close text \textit{pattern}s are dispersed. Thus, %it needs rebalance for overall images, separating the different objects and aggregating homogeneous ones.
%text \textit{pattern}s are not distinct for poor contrast or brightness \etc.
it needs re-balance between \textit{pattern}s (\ie separating the different objects and aggregating homogeneous ones) while maintaining the consistency within each \textit{pattern}. As in Fig.2 (a), text becomes easier to recognize after intensities of `L',`O',`V',`E' and background are pulled away, while the intensities of the characters keep close.
%of poor quality images makes the \textit{pattern}s hard to tell apart.
%the difference and relation between patterns are not clear, so text is not distinctive for visual models. Poor contrast and brightness belong to this case.
(b) \textit{Intra-pattern problem} means text \textit{pattern}s are interfered by the noise like shade, occlusion \etc. As in Fig.2 (b), the shade on left-bottom is mixed with `L', which should be obviated.
%appears when the intended text and unintended interference have similar intensity level, like shade and occlusion, which requires adaptive chromatic intensity adjustment internally within each \textit{pattern}. As in Fig.2(b), the shade on left-bottom corner mixes `L' with the noise, which should be obviated.
} %, and thus generating new \textit{pattern} sets. % to modify the original \textit{pattern}s.
Therefore, a good chromatic rectifier should have the ability to handle with both. % the above two difficulties.
%The difficulty of rectifying chromatic distortions lies in that the chromatic outliers not only contain inconsistent intensities with the normal patterns which can be directly separated by mapping each pixel into a proper intensity space for better brightness or color contrast, but also confusing consistent intensities, which leads to intractable visual inference.

%\textit{Inter-pattern problem} :  it mainly causes quality degenerating in two aspects: 1. invalid and helpful patterns share similar intensity levels, such as low contrast and brightness.    2. helpful patterns are scattered in different intensity levels.  Separating the invalid patterns and Aggregating the helpful ones remain great challenges.
%\textit{Intra-pattern problem} :  where the helpful patterns are interfered by the noise patterns throught shade, occlusion etc.  A compensate mechnism for searching the missing patterns is required.
\begin{figure}[!t]
	\centering
	\includegraphics[scale=0.58]{figure/intro-2-2.jpg}
	\vspace{-0.6cm}
	\caption{Two type of chromatic difficulties. \textit{Pattern} is defined as all the pixels of the same intensity in an image.}
	\label{fig:0-1}
\vspace{-0.6cm}
\end{figure}

In this work,
%In order to handle with both the above two challenges,
we propose a new chromatic rectifier called \textbf{\textit{SPIN}}, which stands for {\textit{\textbf{S}tructure-\textbf{P}reserving \textbf{I}nner Offset \textbf{N}etwork}}. Here, we borrow the concept of \emph{offset} from \cite{MORAN} intended for pixel-level spatial drift at birth, but we enrich it to a broader prospect, containing channel intensity offset (denoted in \textbf{inner offset}) and spatial offset (denoted in \textbf{outer offset}), respectively. The \textit{inner offset} is designed to mitigate chromatic distortions, such as the mentioned \textit{inter-} or \textit{intra-pattern} difficulties, while the \textit{outer offset} incorporates the geometric rectifications such as \cite{RARE,ASTER,MORAN,ESIR,ScRN}. %Specifically,
Note that it is the first to focus on the \textit{inner offset} of scene text,
%as the proposed SPIN restore the shapes of objects while adjusting the intensities for clearer text shape.
as the proposed SPIN mitigates chromatic distortions for clearer shape of object.
{%\color{red}
Specifically, it consists of two components: the \textit{Structure Preserving Network (SPN)} and the \textit{Auxiliary Inner-offset Network (AIN)}. SPN is responsible for alleviating the irregularities caused by \textit{inter-pattern} problems. And AIN is an accessory network to distinguish the irregularities aroused by \textit{intra-pattern} problems.
}
These two components can complement each other. %via an additional \textit{update gate}.
The rectified images will thus become visually clearer for deep networks in intrinsic shape of texts and thus easier to recognize. Moreover, we explore the integration of both the inner and outer offsets by absorbing geometric rectification (\ie TPS \cite{ASTER,wrong}) into SPIN. Experiment verifies that, the unified inner and outer offsets in a single transformation module will assist each other leading to even better recognition.
%{\color{blue}(1. Refer to SR and background removal? 2. color/brightness deviation between vision versus network?)}
The contributions can be summarized as:

(1) To the best of our knowledge, it is the first work to handle with the \textit{chromatic distortions} in STR tasks, rather than the extensively discussed spatial ones. We also introduce the novel concept of \textit{inner} and \textit{outer} offsets in rectification networks and propose a novel SPIN to rectify the images with chromatic transformation.

(2) The proposed SPIN can be easily integrated into deep neural networks and trained in an end-to-end way  without additional annotations and extra losses. Unlike the typical spatial transformation based on STN, which is tied to tedious initialization schemes \cite{RARE,ESIR} or stage-wise training procedures \cite{ScRN}, the SPIN requires \textbf{no} need of sophisticated initialization or any network tricks, which enables it to be a more flexible module.

(3) The proposed SPIN achieves impressive effectiveness in multiple STR tasks. And the combination of chromatic and geometric transformations has been experimentally proved to be practicable and to further outperform existing techniques by a large margin.


==> sections/2_related.tex <==
\vspace{-0.05cm}
\section{Related Work}
\vspace{-0.05cm}
\textbf{{Scene Text Recognition}}. Text recognition in natural scene images is one of the most important challenges in computer vision and various methods have been proposed. Conventional methods were based on hand-crafted features including sliding window methods \cite{SVT,wang-word}, connected components \cite{realtime}, strokelet generation \cite{strokelets}, histogram of oriented gradients descriptors \cite{su2014accurate} \etc. %The Conditional Random Fields (CRF) based methods \cite{shi2013scene} were also proposed in text recognition.
Recent years, deep neural network was dominating the area. %Bissacco \etal \cite{photoocr} applied a network with five hidden layers for character classification.
%Jaderberg \etal \cite{jaderberg2014deep} combined CRF with CNN for unconstrained recognition.
As recurrent neural
networks (RNNs) \cite{LSTM,GRU} were introduced and combined with CNN-based methods\cite{CRNN}, more sequence-to-sequence models \cite{R2AM,FAN,2DCTC,lyu20192d,DAN} were proposed. The attention mechanism was applied to a stacked RNN on top of the recursive CNN \cite{R2AM} and some revisions on the attention \cite{FAN} appeared. Recently, works further advanced the encoder-decoder structure with 2-Dimensional(2-D) ones including 2-D CTC \cite{2DCTC}, 2-D attention \cite{2DATT,lyu20192d} and character-based segmentation before semantic learning \cite{DAN,SRN}.
As modern techniques are powerful to deal with regular texts in scenes, irregular text recognition is still posing a challenging task.
Existing methods include decoder on 2-D featuremaps \cite{2DATT,2DCTC,DAN,SRN}, character-level supervision and guidance \cite{YangX}, generator-based network \cite{Synth}, and rectifications \cite{RARE,ASTER,MORAN,ESIR,ScRN}.
%Among these rectification-based approaches are popular equipped before recognition\cite{RARE,ASTER,MORAN,ESIR,ScRN}, since they do not require any additional annotations or loss functions, flexible yet effective. \cite{wrong,Survey}{\color{red}TO check.}

\vspace{+0.1cm}
\noindent\textbf{{Rectification Network}}.
%As modern techniques are powerful to deal with regular texts in scenes, irregular text recognition is still posing a challenging task.
Among above mentioned approaches handling with \textit{irregularity} of scene texts, rectification-based approaches are popularly equipped before recognition \cite{RARE,ASTER,MORAN,ESIR,ScRN}. % as dominating techniques.
A distinct advantage is that they do not require any additional annotations or loss functions, which is flexible yet effective \cite{wrong,Survey}.
%When it comes to the \textit{irregularity} of scene texts, the dominating techniques are using rectification networks, which is to normalize the input text instance image, remove the distortion, and reduce the difficulty of irregular text recognition \cite{wrong,Survey}.
In this area, all the existing rectifications are limited to the geometric irregularity. Following Spatial Transformer Network (STN) \cite{STN}, RARE \cite{RARE,ASTER} first used thin-plate-spline \cite{TPS} transformation and regressed the fiducial transformation points on curved text. Similarly, ESIR \cite{ESIR} iteratively utilized a new line-fitting transformation to estimate the pose of text lines in scenes, and ScRN \cite{ScRN} improved the control point prediction in STN. MORAN \cite{MORAN} rectified multi-object using predicted offset maps. Different from the image-level rectification, STAR \cite{STAR} proposed a character-aware network by using an affine transformation network to rotate each detected characters into regular ones.
%All the above methods handle with the irregular text using an independent rectification module before recognition to ease the downstream task.
Here, we also work on designing rectification modules to ease the downstream recognition. % since the structure is flexible yet effective to be deployed by any other recognition networks.
%In \textit{decoder-based} type, recent works replace the encoder-decoder structure with 2-D ones including 2-D CTC \cite{2DCTC}, 2-D attention \cite{2DATT,lyu20192d}. The \textit{character-based} methods regard the text recognition as character-aware prediction and then build semantic relation between the independent charaters \cite{xing2019convolutional}. Here, we focus on the first type of network design, since rectification modules are generally more flexible yet effective to be deployed by any other recognition networks.
%The \textit{character-based} methods regard the text recognition as character-aware prediction and then build semantic relation between the independent characters. Here we are focusing on the first type of network design, since rectification modules are generally flexible yet effective to equip with any other recognition networks.
%The first type is to design an independent modules regarded as the pre-preprocessing of the input images without any additional annotations or learning stages by end-to-end training. The latter two kinds are to revise the recognition framework in new proposed encoder-decoders or single character detection at the first step for bypassing the line-based shape irregularity.
%However, when it comes to the \textit{irregularity} of scene texts, all above works are limited by the arbitrary shape.
%Here we are focusing on the first type of network design, since the rectification module is flexible yet effective to equip with any other recognition networks, and does not require any additional annotation by end-to-end training.
%Differently from all the mentioned works \cite{STAR,RARE,ASTER,ESIR,MORAN},
%observing that the challenge of recognition is not only spatial distortions,
Differently from all the existing works, we point out that the \textit{chromatic rectification} is also important. Our proposed network aims to rectify the input patterns from a broader perspective, also handling with the color or brightness difficulties in STR tasks. % while keeping the geometrics-patterns unchanged. %The transformation is robust and flexible in structure distortion estimation and correction.


==> sections/3_methods.tex <==
\section{Methods}
\subsection{Chromatic Transformation}
The proposed chromatic transformation \textit{SPIN}, which stands for Structure-Preserving Inner Offset Network, consists of two components: the Structure Preserving Network (SPN) and the Auxiliary Inner-offset Network (AIN).

\subsubsection{Structure Preserving Network (SPN)}
Inspired by Structure Preserving Transformation (SPT) \cite{SPT}, which cheats modern classifiers by degenerating the visual quality of chromaticity, we find that this kind of distortion is usually fatal to the deep-learning based classifiers. The potential ability of controlling the chromaticity enlightens us to shed light on an even broader application conditioned on proper adaptation. In particular, we find that SPT-based transformations could also rectify the images of color distortions by intensity manipulation, especially for examples like Fig. \ref{fig:0} (c) and (d).
%\noindent\textit{\textbf{Definition 1. Structure Pattern}. Given an image x, the set $\{(i,j)|x(i,j) = c\}$ is called a structure pattern \cite{SPT} with level c.}
Formally, given the input image ${x} \in \mathcal{I}$, let $ x' \in \mathcal{I'}$ denote the transformed image. A transformation $\mathcal{T}$ on $\mathcal{I}$ is defined as follows:
%$$\mathcal{I'}(i,j) = \mathcal{T}[\mathcal{I}(i,j)] \eqno{(1) } $$

$$ x'(i,j) = \mathcal{T}[x(i,j)] \eqno{(1) } $$

where $x(i,j)$ or $x'(i,j)$ is the intensity of the input or output image at the coordinate $(i,j)$. Specifically, the general form of SPT is defined to be a linear combination of multiple power functions:

$$ x'= \mathcal{T}(x)  =  sigmoid( \sum_i \omega_i x^{\beta_i} )  \eqno{(2)}     $$

where $\beta_i$ is the exponent of the i-th basis power function, $\omega_i$ is the corresponding weight. %In general, these exponents can be either learned from data or chosen based on domain knowledge and fixed in advance.
{%Following \cite{SPT} where a group of fixed basis are manually set for simplicity, the empirical formula (3) is applied to calculate $\beta_i$ in pair, where $K$ is the group number of the exponents.
%The empirical formula (3) is applied to calculate $\beta_i$ in pair, where $K$ is the group number of the exponents.
With normalized the intensity of each pixel in [0,1], total intensity space can be scattered into K subspace. Each space can be modeled by an exponential function under certain linear constraint as $y_i = x_i^{\beta_i}$, where $\quad x_i =\frac{i}{2(K+1)}$, $y_i=1-\frac{i}{2(K+1)}$, i=1,2,3,...,K+1.
Then 2K+1 parameters in pair can be formulated as:

$$ \beta_i  = \left\{
\begin{aligned}
& round(\frac{log(1-\frac{i}{2(K+1)} )}{log\frac{i}{2(K+1)}}, 2),  1\leq i  \leq K+1  \\
& round(\frac{1}{\beta_{i-(K+1)}},2),K+1 < i \leq 2K+1.
\end{aligned}
\right.
\eqno{(3)}$$

These $\beta$ exponents can be chosen based on domain or fixed in advance for simplicity.
{%Following \cite{SPT} where a group of fixed basis are manually set for simplicity, the empirical formula (3) is applied to calculate $\beta_i$ in pair, where $K$ is the group number of the exponents.
%The empirical formula (3)
%\cite{SPT}'s chosen set of 11 exponents can be seen as a special instance for $K=5$ in Equa. (3). 
K defines the complexity of transformation intensities. A larger K will support a more complex and fine-grained chromatic space.}
%The calculation can be done efficiently when initialization. Then,
$\omega$ is generated from the input image with convolutional blocks. Therefore, the transformation based on SPN can be summarized as:

$$ x'= \mathcal{T}(x)  =  sigmoid( \sum_i  W^s_{(i)}\mathcal{H_{SPN}}(x) x^{\beta_i} ) \eqno{(4)}   $$

where $W^s$ and $\mathcal{H}_{SPN}(\cdot)$ are part of Block8 weights and the feature extractor, respectively.
$W^s\mathcal{H}_{SPN}(\cdot)$ is a \textit{(2K+1)} dimensional segment from Block8 output of totally \textit{(2K+2)} dimensions, as shown in Fig \ref{fig:1}(a). %The newly proposed transformation can improve the visual quality in an end-to-end trainable way by adjusting the intensities without ruining the structures of the origin images.
\begin{figure*}[!t]
	\centering
	\includegraphics[scale=0.98]{figure/spin-v4.jpg}
	\vspace{-0.3cm}
	\caption{The overview of SPIN. (a) The input image x would first be feed into a well-designed network, and output the updated image x and a group of weights respectively. (b) A structure-preserving transformation is performed on the updated image with the generated weights. } %{\color{red}more vivid details.}
	\label{fig:1}
	\vspace{-0.5cm}
\end{figure*}

\begin{table}[!h]
	\centering
	\scalebox{0.72}{\begin{tabular}{|c|c|c|c|c|}
			\hline
			\multirow{2}{*}{Layers} & \multicolumn{2}{c|}{Configurations}                 &
			\multicolumn{2}{c|}{Output} \\ \cline{2-5}
			%\multirow{2}{*}{Output} \\ \cline{2-3}
			& SPN                      & AIN                      & SPN                     &  AIN                        \\ \hline
			Block1                  & \multicolumn{2}{c|}{Conv(32, 3, 2, 2)}       & \multicolumn{2}{c|}{50$\times$16}                   \\ \hline
			Block2                  & \multicolumn{2}{c|}{Conv(64, 3, 2, 2)}       & \multicolumn{2}{c|}{25$\times$8}                    \\ \hline
			Block3                  & \multicolumn{2}{c|}{Conv(128, 3, 2, 2)}      & \multicolumn{2}{c|}{12$\times$4}                     \\ \hline
			Block4-1/Block4-2       & Conv(256, 3, 2, 2) & Conv(16, 3, 2, 1) & 6$\times$2&6$\times$2                \\ \hline
			Block5-1/Block5-2       & Conv(256, 3, 2, 2)& Conv(1, 3, 1, 1)  & 3$\times$1&6$\times$2                \\ \hline
			Block6                  & Conv(512, 3, 1, 1)  & -                        & 3$\times$1& -                     \\ \hline
			Block7                  & Linear(256)          & -                        & 256 & -                    \\ \hline
			Block8                  & Linear(2K+2)          & -                        & 2K+2 &    -                 \\ \hline
	\end{tabular} }
	\label{tab:1}
    \vspace{-0.1cm}
	\caption{The architecture of SPN and AIN. The parameters in Conv($\cdot$) are filter numbers, kernel, stride and padding size of convolution orderly. For linear blocks, the value in Linear($\cdot$) means output channel numbers. Weights from Block1 to Block3 are sharing.}
	\vspace{-0.2cm}
\end{table}

\iffalse
\begin{table*}[!h]
	\centering
	\scalebox{0.85}{\begin{tabular}{|c|c|c|c|c|}
			\hline
			\multirow{2}{*}{Layers} & \multicolumn{2}{c|}{Configurations}                 &
			\multicolumn{2}{c|}{Output} \\ \cline{2-5}
			%\multirow{2}{*}{Output} \\ \cline{2-3}
			& SPN                      & AIN                      & SPN                     &  AIN                        \\ \hline
			Block1                  & \multicolumn{2}{c|}{3$\times$3 Conv, 32, k:2$\times$2, s:2$\times$2}       & \multicolumn{2}{c|}{50$\times$16}                   \\ \hline
			Block2                  & \multicolumn{2}{c|}{3$\times$3 Conv, 64, k:2$\times$2, s:2$\times$2}       & \multicolumn{2}{c|}{25$\times$8}                    \\ \hline
			Block3                  & \multicolumn{2}{c|}{3$\times$3 Conv, 128, k:2$\times$2, s:2$\times$2}      & \multicolumn{2}{c|}{12$\times$4}                     \\ \hline
			Block4-1/Block4-2       & 3$\times$3 Conv, 256, k:2$\times$2, s:2$\times$2 & 3$\times$3 Conv, 16, k:2$\times$2, s:1$\times$1 & 6$\times$2&6$\times$2                \\ \hline
			Block5-1/Block5-2       & 3$\times$3 Conv, 256, k:2$\times$2, s:2$\times$2 & 3$\times$3 Conv, 1               & 3$\times$1&6$\times$2                \\ \hline
			Block6                  & 3$\times$3 Conv, 512             & -                        & 3$\times$1& -                     \\ \hline
			Block7                  & Linear, 512, 256          & -                        & 256 & -                    \\ \hline
			Block8                  & Linear, 256, 2K+2          & -                        & 2K+2 &    -                 \\ \hline
	\end{tabular} }
	\label{tab:1}
	\caption{The architecture of SPN and AIN. The parameters in Conv(\cdot) are filter numbers, kernel, stride and padding size of convolution orderly. For linear blocks, the value in Linear(\cdot) means output channel numbers. Weights from Block1 to Block3 are sharing. }
	\vspace{-0.5cm}
\end{table*}
\fi
In essence, \textbf{Structure-Preserving} is realized by filtering the intensity level of input images.
All the pixels with the same intensity level in the original image have the same intensity level in the transformed image, where the set $\{(i,j)|x(i,j)=c\}$ with intensity level c is defined as \textit{structure-pattern}s. Intuitively, we propose the SPN for rectifying chromatic distortions by taking advantage of this singleton-based pixel-wise transformation in \textit{two aspects}:  (1) Separating useful structure-patterns from the harmful ones by injecting them to different intensity levels, which will be likely to generate better contrast and brightness. (2) Aggregating different levels of structure-patterns by mapping them to close intensity levels, which will be beneficial to alleviate fragments, rendering a more unified image. These are suitable for handling with \textit{inter-pattern} problems (as Fig.2 (a)) but powerless against the other.
\vspace{-0.1cm}
\subsubsection{Auxiliary Inner-offset Network (AIN)}
\label{ION}
Since SPN tries to separate and aggregate the specific \textit{structure-pattern}s by exploiting the spatial invariance of words or characters, it inexplicably assumes that these patterns are under inconsistent intensities, namely different levels of \textit{structure-pattern}s. However, it does not consider the disturbing patterns can have similar intensity with the useful ones, noted as \textit{pattern confusion}, causing \textit{intra-pattern} problems (as Fig.2 (b)). %In fact, these patterns will have no chance to be separated due to the intrinsic property of SPN. % and may also degenerate visual quality.

To handle with the difficulty, we borrow the concept of \emph{offset} from geometric transformation \cite{MORAN} while we decouple geometric and chromatic offsets for better understanding of the rectification procedures. SPN will generate \textbf{chromatic offsets}(namely \textit{inner-offsets}) on each coordinate. As mentioned above, solely SPN is limited by the intrinsic \textit{pattern confusion} problems. Here, we design an auxiliary inner-offset network (AIN) to assist with the consistent intensity for patterns. The \textit{auxiliary inner-offset} is defined as:
%\begin{equation}
\iffalse
$$
\begin{aligned}
\hat{x}(i,j) &= g(x(i,j)) \\
   &= (1-\alpha) \circ x(i,j) + \alpha \circ x_{\text{offsets}}(i,j)
\end{aligned} \eqno{(5)}
$$
\fi

$$g(x) = (1-\alpha) \circ x + \alpha \circ x_{\text{offsets}} \eqno{(5)}$$

%\end{equation}
%$$ \hat{x}(i',j')= g(\mathcal{S}(x, f(i', j'))) = g(\mathcal{S}(x,(i',j'))) = g(x(i',j'))  \eqno{(6)}$$
%defined as:
%$$ g(x(i,j)) = (1-\alpha) \circ x(i,j) + \alpha \circ x_{\text{offsets}}(i,j) \eqno{(7)} $$
%where
where

$$ \alpha = sigmoid(W^z \mathcal{H_{SPN}}(x))  \eqno{(6)} $$
$$ x_{\text{offsets}} = W^a \mathcal{H_{AIN}}(x). \eqno{(7)}$$

$W^z$ is the trainable scalar which is partial output from Block8 in Fig \ref{fig:1}(a). Similarly, $W^a$ is the trainable parameter in AIN module and $\mathcal{H_{AIN}}(\cdot)$ is feature extractor sharing the first 3 blocks with SPN. $\circ$ is hadamard product. We design a learnable update gate $\alpha$, which can receive signals from SPN and perceive the difficulty of different tasks. It is responsible for controlling the balance between the input image x and the predicted auxiliary inner-offsets. $g(x)$ (or $x$) is the updated (or input) image. Here, $x_{\text{offsets}}$ is predicted by AIN, whose architecture is also given in Table 1.
As chromatic transformation is pixel-to-pixel mapping on each coordinate and thus requires no need of spatial shift. The AIN first divides the image into small patches and then predicts offsets for each. All the offset values are activated by $sigmoid(\cdot)$ and mapped into the size of input image via common upsampling (\eg{bilinear interpolation}). % or up-sampling operation on warped images.
%$f$ is set to be the identity function and thus requires no need of sampling operation.
The auxiliary inner-offsets can mitigate the \textit{pattern confusion} through slight intensity-level perturbations $x_{\text{offsets}}(i,j)$ on each coordinate $(i,j)$.
%The AIN first divides the image into small patches and then predicts offsets for each. All the offset values are activated by $Sigmoid(\cdot)$ and mapped into the size of input image via bilinear interpolation.
Assisted by AIN, the enhanced transformation will be performed on the updated images, and the comprehensive transformation $\hat{\mathcal{T}}$ can be formulated upgrading Equa. (2) by
%$$\mathcal{SPIN}_{i,j}(x)  =  sigmoid( BN(\sum_t \omega_t (\mathcal{O}_{i,j}(x) )^{\beta_t}) ). \eqno{(9)}$$
%\hat{x'}

$$\hat{x'} =  \hat{\mathcal{T}}(x)  =  sigmoid( \sum_i \omega_i (g(x))^{\beta_i} ) \eqno{(8)}$$

%Note that the transformation manipulates the intensity without ruining the structure-patterns all the time.
The detailed network and the overall structure are also illustrated in Table 1 and Fig. \ref{fig:1}.
\vspace{-0.1cm}
\subsection{Geometric-Absorbed Extension}
Spatial transformations \cite{STAR,RARE,ASTER,ESIR,MORAN} rectify the location shift of patterns by predicting the corresponding coordinates, which will generate geometric offsets (namely \textit{outer-offset}s). And then they re-sample the whole images based on the points, which could be described as:

$$ \tilde{x'}(i',j')= \mathcal{S}(x, f(i', j'))=\mathcal{S}(x, (i, j))  \eqno{(9)}$$
%$$ x'(i',j')= \mathcal{S}(x, f(i', j')),  f: (i',j') \longmapsto (i,j)  \eqno{(9)}$$

where $(i,j) (or (i',j'))$ is the origin coordinate (or the coordinate adjusted by outer-offsets), $\mathcal{S}(x,\cdot)$ here stands for the sampler, which generates the transformed images by interpolating the neighbor pixels in $x(i,j)$, and $f$ represents different forms of  transformation function, \eg Affine \cite{STAR,RARE}, Thin-Plate-Spline(TPS) \cite{TPS,RARE,ASTER,ScRN}, Line-Fitting Transformation \cite{ESIR}.
%Differently, SPT will generate chromatic offsets (namely \textit{inner-offsets}) on each coordinate. As mentioned above, solely SPT is limited by the intrinsic problems of \textit{pattern coherence}. Here, we design an auxiliary innet-offset network (AIN) to assist the main transformation to handle with the consistent intensity for texts. The auxiliary offsets are defined as:
Differently, in the proposed chromatic transformation generate \textit{inner-offsets} on each coordinate as Equa. (1). Both are independent modules used to ease downstream stages, while they can be integrated as the unified transformation as

%$$ \mathcal{\hat{I'}}(i',j')=\mathcal{T}[\mathcal{I}(i',j')]= \mathcal{T}[g(\mathcal{S}(x, f(i', j')))] \eqno{(11)}$$ % = g(\mathcal{S}(x,(i',j')))
$$ \begin{aligned}
\ddot{x'}(i',j')&= \mathcal{S}(\hat{x'}, f(i', j')) \\
&= \mathcal{S}(\hat{\mathcal{T}}(x),  f(i', j')).
\end{aligned}
\eqno{(10)}
$$ % = g(\mathcal{S}(x,(i',j')))

We call the uniform of chromatic and geometric rectification as Geometric-Absorbed SPIN (short in \textit{GA-SPIN}).
Note that the learnable parameters in both chromatic transformation $\hat{\mathcal{T}}(\cdot)$ and geometric transformations $f(\cdot)$ are simultaneously predicted by the unified network configurations in Table 1. When absorbing spatial rectifications like TPS, the only difference for GA-SPIN compared to SPIN is the output channel numbers of Block8 are set to $2K+2+N$ instead of $2K+2$, as N is number of parameters for TPS (\eg 40).
\vspace{-0.1cm}
\subsection{Recognition Network and Training}
For direct comparison on rectification, we adopt the mainstreaming recognition network \cite{wrong} and all its configuration and setups. %, which consists of four-stage recognition pipeline: Transformation, Feature Extraction,  Sequence Modeling and Prediction. The \textit{Transformation} network rectifies an input image with predicted transformation parameters to ease downstream stages. And the last three stages are widely-used regular text recognition network.
%\textit{Feature Extraction} network will map the input image to a compact representation. The \textit{Sequence Modeling} captures the contextual information and the \textit{Prediction} modules map the identified representation into final characters.
Specifically,
%to build encoders including Feature Extraction and Sequence Modeling modules,
for contextual feature, we use typical STR backbones of 7-layer of VGG \cite{VGG} or 32-layer ResNet \cite{ResNet} with two layers of Bidirectional long short-term memory (BiLSTM) \cite{LSTM} each of which has 256 hidden units as \cite{CRNN,FAN}.
%the setting of CRNN \cite{CRNN} and FAN \cite{FAN} are selected. The typical network consists of a 7-layer of VGG \cite{VGG} or 32-layer ResNet \cite{ResNet} and two layers of Bidirectional long short-term memory (BiLSTM) \cite{LSTM} each of which has 256 hidden units.
Following \cite{wrong}, the decoder adopts an attentional LSTM with 256 hidden units, 256 attention units and 69 output units (26 letters, 10 digits, 32 ASCII punctuation marks and 1 EOS symbol).
%Our model is fully end-to-end trainable by minimizing the conventional loss function on the recognition output probabilities.
%During the inference stage, we directly select the most probable characters. Only digits and letters are counted and the rest is discarded.
%{\color{red}TO strenghen fairness}


==> sections/4_exp.tex <==
\vspace{-0.1cm}
\section{Experiments}
%{In this section we describe extensive experiments in evaluation of each modules in the proposed method, and then compare the performance with other state-of-the-art methods. We conducted on various benchmarks, including both regular and irregular datasets. The performances of all the methods are measured by word accuracy.}
\begin{table*}[!htb]
	\centering
	\scalebox{0.88}{
		\begin{tabular}{|p{1.5cm}<{\centering}|l|*{2}{p{0.7cm}<{\centering}}|*{7}{p{0.75cm}<{\centering}}|p{0.8cm}<{\centering}|}
			\hline
			\multicolumn{1}{|c|}{\multirow{2}{*}{Rectification}} &
			\multicolumn{1}{c|}{\multirow{2}{*}{Transformation}} & \multicolumn{2}{c|}{Offsets}        & \multicolumn{8}{c|}{Benchmark}     \\ \cline{3-12}
			\multicolumn{1}{|c|}{}   &  \multicolumn{1}{c|}{}                           & \multicolumn{1}{c}{Outer} & Inner & IIIT                 & SVT                  & IC03                 & IC13                 & IC15                 & SVTP                 & CT                  & \multicolumn{1}{c|}{ Avg}         \\ \hline
			None &(a) \footnotesize{None$^\dagger$ \cite{RARE}  }                                             & No                         & No    &      82.4                &     81.9                 &   91.2                   &   87.3                   &   67.4                   &  70.9                    &   61.6                    &   77.5            \\ \hline
			\multirow{2}{*}{Chromatic} &(b) \footnotesize{SPIN w/o AIN }                                            & No                         & Yes    &
			82.1                   &   84.2                  &   91.9                &  87.8                   &        67.3                   &   72.3                   &  63.5                 &   78.4                   \\
			%(c) \footnotesize{+ Scheme Initialization}                                            & No                         & Yes   &
			%82.5                    &   82.8                &  91.2                   &   87.9                   &  67.3                    &   74.1                   &   63.9                    &   78.5             \\
			&(c) \footnotesize{SPIN}                                           & No                         & Yes   &   82.3                   &   84.1                  &  91.6                    &    88.7                  &   68.1                   &    72.3                  &   64.6                    &    78.8                 \\\hline
			Geometric &(d) \footnotesize{STN$^\dagger$ \cite{wrong}}                                      & Yes                        & No    & \multicolumn{1}{c}{82.7} & \multicolumn{1}{c}{83.3} & \multicolumn{1}{c}{92.0} & \multicolumn{1}{c}{88.5} & \multicolumn{1}{c}{69.6} & \multicolumn{1}{c}{74.1} & \multicolumn{1}{c|}{62.9} & \multicolumn{1}{c|}{79.0}  \\\hline
			\multirow{2}{*}{Both} &(e) \footnotesize{SPIN+STN }                                            & Yes                        & Yes   &  83.6                    &   84.4                   &   92.7                   &  89.2                    &  70.9                    &   73.2                   &   64.6                    &  79.8                     \\ %\hline
			&(f) \footnotesize{GA-SPIN}     & Yes & Yes & 84.1 &83.2 &92.3&88.7&71.0&74.5&67.1&80.1 \\\hline
		\end{tabular}
	}
    \vspace{-0.1cm}
	\caption{Comparison between the baseline and the model combined with different rectifications. All the models are evaluated based on accuracy under several benchmarks. The `Offset' stands for enabling the corresponding offset modules. `$\dagger$' indicates the model is tested by us under a fair setting.} %}
    \vspace{-0.1cm}
	\label{table:2}
\vspace{-0.3cm}
\end{table*}

\subsection{Dataset}
%All the models are trained on 2 synthetic datasets and evaluated over 7 widely used benchmarks listed as follows. %, and all these datasets have been widely used.
Models are trained only on 2 public synthetic datasets MJSynth (MJ) \cite{MJ} and SynthText (ST) \cite{ST} without any additional dataset or data augmentation.
We evaluate on 4 regular and 3 irregular datasets as follows according to the difficulty and geometric layout of the text \cite{wrong}.
%Following formerly unified settings for text recognition \cite{wrong}, we use 2 synthetic datasets for training, including  \textbf{MJSynth (MJ) }\cite{MJ} which contains 9 million synthetic text images and \textbf{SynthText (ST)} \cite{ST} where we crop 7 million text image patches from original images for detection.

%The popular benchmarks were categorized into 4
%regular and 3 irregular datasets as follows according to the difficulty and geometric layout of the texts. %The regular cases are relatively easy for STR models:

\noindent \textbf{IIIT5K (IIIT)} \cite{IIIT5K} contains scene texts and born-digital images. It consists of 3,000 images for evaluation.

\noindent \textbf{SVT} \cite{SVT} contains 647 images for evaluation, collected from Google Street View, some of which are noisy, blurry, or of low-resolution.

\noindent \textbf{ICDAR2003 (IC03)} \cite{IC03} contains 860 images for evaluation which was used in the Robust Reading Competition in the International Conference on Document Analysis and Recognition (ICDAR) 2003.

\noindent \textbf{ICDAR2013 (IC13)} \cite{IC13} contains 1015 for evaluation which was used in the ICDAR 2013.

%The irregular cases are relatively hard for STR models, usually contain cases such as curved, blurry, and occlusion.
\noindent \textbf{ICDAR2015 (IC15)} \cite{IC15} contains 2,077 text image patches are cropped scene texts suffer from perspective and curvature distortions, which was used in the ICDAR 2015. Researchers have used two different versions for evaluation: 1,811 and 2,077 images. %Some extremely geometrically distorted images were discarded in the 1,811 version.
We use 1,811 images in our discussions and report both results when compared with other techniques for fair comparisons.
%Following \cite{FAN}, the dataset is filtered by discarding words that contain non-alphanumeric characters and some extremely rotated, perspective-shifted, and curved images for evaluation.

\noindent \textbf{SVTP} \cite{SVTP} contains 645 images for evaluation. Many of the images contain perspective projections due to the prevalence of non-frontal viewpoints.

\noindent \textbf{CUTE80 (CT)} \cite{CUTE80} has 288 cropped images for evaluation. Many of these are curved text.
%claimed in \cite{wrong} that it is hard to assess whether and how a newly
%proposed module improves upon the current art, as some papers have come up with different evaluation and testing environments.
%Note that models will be trained on the MJSynth dataset by default. For fair comparison, the SynthText dataset will be used under the state-of-the-art settings. All experiments are only with word-level annotations and there is no fine-tuning stage or adding any extra private dataset.
%Section \ref{ION} gives the definitions of the \textit{Outer} and \textit{Inner}, which refes to geometric and spatial-invariance offsets, respectively.
\vspace{-0.1cm}
\subsection{Implementation}
All images are resized to 32 $\times$ 100 before entering the network. $K=6$ is the default setting. The parameters are randomly initialized using He \etal's method \cite{He} if not specified. Models are trained with the AdaDelta \cite{adadelta} optimizer for 5 epochs with batch size = 64.
%Gradient clipping is used at magnitude 5.
The learning rate is set to 1.0 initially and decayed to 0.1 and 0.01 at 4-th and 5-th epoch, respectively.

\textbf{NOTE} that the inconsistent choices of datasets, network and training configurations make fair comparison and module-wise assessment of recent works more difficult. We evaluate the proposed rectification module with SOTAs rigorously using the same datasets, recognition network and training setups as the unified benchmark \cite{wrong}. All experiments are only with word-level annotations. The network is trained from the scratch end-to-end without stage-wise procedures or other tricks.
\vspace{-0.1cm}
\subsection{Effects of Rectification Module}
To go deep into individual factors in the proposed model, we cumulatively enable each configuration \textit{one-by-one} on top of a solid baseline. All models are trained on the MJ dataset with backbone of 7-layer VGG. Following models are all the same by default. Table \ref{table:2} lists the accuracy in each configuration.
\vspace{-0.1cm}
\subsubsection{Chromatic Transformation.}
The item (a) poses the baseline \cite{RARE} without the rectification module. (b) and (c) add the rectification module and verify the advantage of the chromatic rectification. Specifically, (b) enables the proposed SPIN w/o AIN and improves (a) by an average of 0.9\%. And (c) moves forward to enable AIN with SPN, composing SPIN. Though only two additional convolution layers appended to (b), (c) obtains an average of 0.4\% consistent improvement and a total of 1.2\% improvement compared with the baseline. The enhancement is mainly from SVT, IC15 and CUTE80, where lots of images with chromatic distortions are included. In addition, the first 3 rows in Fig. 5, mostly the \textit{inter-pattern} distortions are transformed to clearer shape through SPIN-based method, and the last row, seemingly the \textit{intra-pattern} problems(\ie shadow), also show the obvious effect between SPIN over w/o AIN.
\vspace{-0.1cm}
\subsubsection{Chromatic versus Geometric Transformation.}
%As mentioned, all existing rectification modules are focused on geometric transformations, as
Table 2(d) shows the baseline (a) equipped with STN \cite{wrong}, which rectifies images via \textit{outer-offset}s and achieved superior performance among the state-of-the-arts. Interestingly, the performance of SPIN in (e) is close to that of the geometric one. The difference lies in that, the former mainly improves the SVT and CUTE80 benchmarks, where large proportion of chromatically distorted images are included, while the latter mainly improves the IC15 and SVTP benchmarks, where rotated, perspective-shifted and curved images dominate. And it verifies the color rectification is comparably important with shape transformation and the two type of rectifiers possess their respective strengths.
\vspace{-0.1cm}
\subsubsection{Combining Chromatic and Geometric Transformation.}
%We then explore the combination of both geometric and chromatic rectifications.
We further explore whether inner-offsets assist the existing outer-offsets \cite{RARE} and how these two categories can jointly work better.
In (e), simply placing the SPIN (c) before the TPS-based STN (d) (denoted as \textit{SPIN+STN}) without additional modification brings an average of 0.8\% improvement, compared with configuration (d).
%The data flow in the forward pass of the rectification module is as follows: $\mathcal{I} \rightarrow SPIN(\cdot) \rightarrow STN(\cdot) \rightarrow \mathcal{I'}$, where $SPIN(\cdot)$ and $STN(\cdot)$ represents the two complete operation performed by two independent networks.
%An average of 0.8\% improvement, compared with configuration (d), can be directly achieved,
It indicates that these two transformations are likely to be two complementary strategies, where the inner part was usually ignored by the former researchers.
%As the pipeline of SPIN and STN is verified beneficial in accuracy in (e) while brings additional computational cost and superfluous parameters. %To explore the problems ulteriorly,
GA-SPIN in (f) unifies SPIN and TPS-based STN in a single transformer (illustrated in Section 3.2).
%In detail, two types of offset are integrated together, where the parameters of the inner and outer offset are simultaneously predicted by one single network, no longer from two separate modules.
%The geometric and chromatic parts share the same convolution network, and differ only in output channels of the last linear layer. For instance, the output channel number for SPN is 2K+2 as illustrated in Table 1., and for GA-SPIN the number is 2K+2+N, only additional N outputs (N is number of the parameters for localization in TPS, \eg 40).
Though cutting parameters and computation cost compared to the straightforward pipeline structure (e), it improves the results by 0.3\% on average and gains a large margin by 1.1\% compared to solely geometric transformers (d). It means GA-SPIN is a simple yet effective integration. % of the two kinds. %and the different types of rectifications truly complement each other.
%Note that despite TPS, other kinds of spatial transformers (\eg, Affine \cite{STAR}, MORN \cite{MORAN} ) can also be easily extended with our proposed SPIN using methods in either (e) or (f) similarly.
%\vspace{-0.5cm}
\subsection{Discussion}
\subsubsection{Discussion on Sensitivity to Weight Initialization.} Proper weight initialization is necessary for geometric transformations \cite{RARE,ASTER,ESIR}, since highly geometrically distorted images will ruin the training of the recognition network.
%Thus we have to follow the scheme proposed by Shi \etal \cite{RARE} for all the \textit{TPS} transformations in this paper.
On the contrary, chromatic transformations are less likely to severely distort the images for the intrinsic merits of preserving the \textit{structure-pattern}s. Random initialization works well in Table \ref{table:2} (b) and (c), indicating insensitivity to weight initialization of our modules.
%However, we observed convergence failure when geometric transformations are included, which proves that the severe chromatic distortions do affect the performance of geometric rectification. For a better flexibility adapted with other structures requiring careful parameters, we initialize the last fully-connected layer of SPIN with zero weights and biases of certain values. The values, which are all set to zero except the ones corresponding to exponent = 1.00 and the update gate are set to 1.0 and -1.0, respectively.
\begin{figure}[!htb]
    \vspace{-0.4cm}
	\centering
	\includegraphics[scale=0.33]{figure/discuss_k_hor.pdf}
	\vspace{-0.6cm}
	\caption{Results on different K. All the models are trained on the MJ dataset using VGG feature extractor. The line in coral, blue and red refer to the baseline without rectification module, with SPIN and with GA-SPIN, respectively. The results are evaluated with the mean accuracy.}
% of 4 regular benchmarks and 3 irregular benchmarks.}
	\label{fig:3}
\end{figure}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
%\vspace{-0.2cm}
\begin{table}[!b]
    \vspace{-0.2cm}
	\centering
	\scalebox{0.78}{
%\begin{tabular}{p{4.2cm}<{\centering}|{p{1.9cm}<{\centering}}|{p{1.9cm}<{\centering}}|{p{1.9cm}<{\centering}}|p{1.1cm}<{\centering}}
		\begin{tabular}{|c|c|c|c|c|} %{|l|l|l|*{8}{p{0.8cm}<{\centering}}|}
        \hline
		\multirow{2}{*}{Transformation} & \multicolumn{3}{c|}{Accuracy(\%)}& \multirowcell{2}{$\#$Para.\\($\times 10^6$)} \\ \cline{2-4}
        &VGG-MJ & ResNet-MJ& ResNet & \\ \hline
		None     & 66.6          &  69.0  & 74.9 &0 \\
		STN \shortcite{wrong}$^\dagger$   & 68.9(+2.3)   &  71.2(+2.2)&76.9(+2.0) & 1.68 \\
		
		ASTER \shortcite{ASTER}            & 68.2(+1.6) &  70.6(+1.6)$^*$ &78.0(+3.1)$^*$ &  - \\
		ESIR \shortcite{ESIR}                  & 70.2(+3.6)   &  72.7(+3.7)$^*$ &79.9(+5.0)$^*$ &  -   \\
        ScRN \shortcite{ScRN}                  & -    & \textbf{73.0(+4.0)}$^*$ & 82.3(+7.4)$^*$ & 2.62 \\
		\hline

		%SPIN w/o AIN                          & 67.7(+0.9)   & 69.9(+0.9) &- &2.28 \\
		SPIN                           & 68.3(+1.7)   &  71.0(+2.0)  &81.3(+6.4) &2.30\\
	    GA-SPIN               & \textbf{70.9(+4.3)} & \textbf{73.0(+4.0)} & \textbf{84.5(+9.6)}& 2.31 \\ \hline
	\end{tabular}
	}
	\vspace{-0.1cm}
	\caption{Comparison with rectification methods. The values are mean accuracy of 3 irregular benchmarks. `-MJ' means only using MJ dataset. `*' denotes the results with deeper 45/50-layer than our 32-layer ResNet setting. `$\dagger$' indicates the model is tested by us under the same setting for fairness.}
\label{table:2.1}
\vspace{-0.3cm}
\end{table}


\iffalse
\begin{table*}[!b]
	\centering
	\scalebox{0.9}{
\begin{tabular}{p{4.2cm}<{\centering}|*{2}{p{1.9cm}<{\centering}}|*{2}{p{1.9cm}<{\centering}}|*{2}{p{1.9cm}<{\centering}}|p{1.1cm}<{\centering}}
		\hline
		\multirow{2}{*}{Transformation} & \multicolumn{2}{c|}{Accuracy (VGG)} & \multicolumn{2}{c|}{Accuracy (ResNet)} &  \multicolumn{2}{c|}{Accuracy (ResNet)} & \multirowcell{2}{$\#$Para.\\($\times 10^6$)} \\ \cline{2-7}
		& Regular(\%)    & Irregular(\%)   & Regular(\%)     & Irregular(\%)  & Regular(\%)     & Irregular(\%)    &                        \\ \hline
		None \cite{RARE}$^\dagger$              & 85.7        & 66.6             &  86.5  &  69.0   &  & &0 \\
		TPS-STN \cite{wrong}$^\dagger$  & 86.6(+0.9)   & 68.9(+2.3)   & 87.1(+0.6)  &  71.2(+2.2) &90.6&74.5 & 1.68 \\
		
		ASTER \cite{ASTER}            & 87.0(+1.3)   & 68.2(+1.6)   & \textbf{88.2(+1.7)}$^*$ &  70.6(+1.6)$^*$   & 92.3  &78.0 &  - \\
		ESIR \cite{ESIR}              & -            & 70.2(+3.6)   &   -  &  72.7(+3.7)$^*$   &- &79.9$^*$ &  -   \\
        ScRN \cite{ScRN}              & -            & -   &   -  &  -   & 93.1 & 82.3 & 2.62 \\
		\hline

		SPIN w/o AIN                           & 86.5(+0.8)   & 67.7(+0.9)   &  87.5(+1.0)  & 69.9(+0.9)    &- &- &2.28 \\
		SPIN                         & {86.7(+1.0)}   & 68.3(+1.7)   & 87.6(+1.1) &  71.0(+2.0)  & 91.8 &81.3 &2.30\\
	    {GA-SPIN}              & \textbf{87.1(+1.4)}  & \textbf{70.9(+4.3)} & 87.8(+1.3) & \textbf{73.0(+4.0)}  & 93.1& 84.2& 2.31 \\ \hline
	\end{tabular}
	}
	\caption{Comparison with SOTA rectification networks. The accuracies are acquired by taking the mean of the results of the regular and irregular benchmarks including that module respectively. `*' denotes the reported results are using deeper 45-layer ResNet than our basic 32-layer ResNet setting. `$\dagger$' indicates the model is tested by us under the same setting.}
\label{table:2.1}
\end{table*}
\fi

\iffalse
\begin{table*}[!b]
	\centering
	\scalebox{0.9}{
	\begin{tabular}{p{4.2cm}<{\centering}|*{2}{p{1.9cm}<{\centering}}|*{2}{p{1.9cm}<{\centering}}|p{1.1cm}<{\centering}}
		\hline
		\multirow{2}{*}{Transformation} & \multicolumn{2}{c|}{Accuracy (VGG)} & \multicolumn{2}{c|}{Accuracy (ResNet)} & \multirowcell{2}{$\#$Para.\\($\times 10^6$)} \\ \cline{2-5}
		& Regular(\%)    & Irregular(\%)   & Regular(\%)     & Irregular(\%)     &                        \\ \hline
		None \cite{RARE}$^\dagger$              & 85.7        & 66.6             &  86.5  &  69.0   & 0  \\
		TPS-STN \cite{wrong}$^\dagger$  & 86.6(+0.9)   & 68.9(+2.3)   & 87.1(+0.6)  &  71.2(+2.2) & 1.68 \\
		
		ASTER \cite{ASTER}            & 87.0(+1.3)   & 68.2(+1.6)   & \textbf{88.2(+1.7)}$^*$ &  70.6(+1.6)$^*$   &  -    \\
		ESIR \cite{ESIR}              & -            & 70.2(+3.6)   &   -  &  72.7(+3.7)$^*$   &  -    \\
		\hline
		SPIN w/o AIN                           & 86.5(+0.8)   & 67.7(+0.9)   &  87.5(+1.0)  & 69.9(+0.9)    & 2.28 \\
		SPIN                         & {86.7(+1.0)}   & 68.3(+1.7)   & 87.6(+1.1) &  71.0(+2.0)  & 2.30 \\
	    {GA-SPIN}              & \textbf{87.1(+1.4)}  & \textbf{70.9(+4.3)} & 87.8(+1.3) & \textbf{73.0(+4.0)}  & 2.31 \\ \hline
	\end{tabular}
	}
	\caption{Study of modules with respect to accuracy and the number of parameters. The accuracies are mean of the results of the regular and irregular benchmarks including that module respectively. `*' denotes the reported results are using deeper 45-layer ResNet than our basic 32-layer ResNet setting. `$\dagger$' indicates the model is tested by us under the same setting.}
\label{table:2.1}
\end{table*}
\fi
\begin{figure}[!t]
	\centering
	\includegraphics[scale=0.5]{figure/effect_1-4.jpg}
    \vspace{-0.5cm}
    \caption{Visualization of rectification with chromatic problems, unbalanced contrast (row 1-2), low brightness (row 3) and shadow (row 4),respectively. Samples here and in Fig. \ref{fig:5} are all from SVT, IC15 and CUTE80 test sets.}
	%\caption{Visualization of rectification with chromatic problems. Samples are from IC15 and CUTE80. The first 3 rows are mainly with \textit{inter-pattern} problems and the last poses \textit{intra-pattern} challenge.}
	%\caption{Visual comparison of different rectification methods: the input images are in the first column, columns 2-4 show the rectified images by using the TPS-based STN, SPIN, and GA-SPIN, respectively. The sample images are from IC15 and CUTE80. The proposed SPIN performs better in chromatic distortion rectification and GA-SPIN performs well on both geometric and chromatic distortion rectification.}
	\label{fig:4}
    \vspace{-0.3cm}
\end{figure}
\vspace{-0.3cm}
\begin{figure}[!t]
	\centering
	\includegraphics[scale=0.6]{figure/effect_2-3.jpg}
	\vspace{-0.1cm}
	\caption{Examples of the rectification effects and prediction. ``gt'' is the ground truth. Predictions are shown under the images. Red are mistakenly recognized characters. } %Samples are from SVT, IC15 and CUTE80.}
	\label{fig:5}
    \vspace{-0.5cm}
\end{figure}

\vspace{-0.1cm}
\begin{table*}[!t]
	\centering
	\scalebox{0.75}{
		\begin{tabular}{|l|l|l|l|l|*{8}{p{0.8cm}<{\centering}}|}
			\hline
			\multirow{2}{*}{Methods}  & \multirow{2}{*}{Rect}& \multirow{2}{*}{ConvNet} & \multirow{2}{*}{Training data} & \multirow{2}{*}{Supervision} & \multicolumn{8}{c|}{Benchmark}                                                                                                                                                  \\ \cline{6-13}
			&                          &    &              &              & IIIT                  & SVT                      & IC03                     & IC13                     & IC15a & IC15b                  & SVTP                  & CT                   \\ \hline
			Jaderberg \etal \cite{JaderbergReading}         &      & VGG                      & MJ            &   Word       & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{80.7} & \multicolumn{1}{c}{93.1} & \multicolumn{1}{c}{90.8} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c|}{-} \\
			Shi \etal \cite{CRNN}             &        & VGG                      & MJ          &   Word                   & 78.2                  & 80.8                     & 89.4                     & 86.7                     & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c|}{-} \\
			Shi \etal \cite{RARE}      &$\surd$              & VGG                      & MJ          &      Word              & 81.9                  & 81.9                     & 90.1                     & 88.6                     & \multicolumn{1}{c}{-} &    \multicolumn{1}{c}{-} & 71.8                  & 59.2                   \\
			Lee \etal  \cite{R2AM}          &        & VGG                      & MJ             &   Word                & 78.4                  & 80.7                     & 88.7                     & 90.0                     & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} &  \multicolumn{1}{c|}{-} \\
			%Yang \etal \cite{Yang}             & VGG                      & P         &    Word+Char            & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-}    & \multicolumn{1}{c}{-}    & \multicolumn{1}{c}{-}    & \multicolumn{1}{c}{-} &  \multicolumn{1}{c}{-}   & 75.8              & 69.3                   \\
			%Cheng \etal \cite{AON}   & VGG                   & MJ+ST        &    Word            & 87.0        & 82.8                     & 91.5                     &  \multicolumn{1}{c}{-}                     & - &   \multicolumn{1}{c}{68.2} &  73.0         & 76.8 \\			
			
			
			%Liu \etal \cite{STAR}        &         & ResNet                   & MJ+P      &     Word             & 83.3                  & 83.6                     & 89.9                     & 89.1                     & \multicolumn{1}{c}{-}  & \multicolumn{1}{c}{-} &  73.5                  & \multicolumn{1}{c|}{-} \\
					
			%\hline
			%Shi \etal \cite{CRNN} *                     & VGG                      & MJ+ST                          & 82.9                  & 81.6                     & 93.1                     & 89.2                     & 69.4                  & 70.0                  & 65.5                   \\
			%Shi \etal \cite{RARE} *                    & VGG                      & MJ+ST                          & 86.2                  & 85.8                     & 93.9                     & 91.1                     & 74.5                  & 76.2                  & 70.4                   \\
			%Lee \etal \cite{R2AM} *                 & VGG                      & MJ+ST                          & 83.4                  & 82.4                     & 92.2                     & 88.1                     & 68.9                  & 72.1                  & 64.9                   \\
			%Liu \etal \cite{STAR} *                 & ResNet                   & MJ+ST                          & 87.0                  & 86.9                     & 94.4                     & 91.5                     & 76.1                  & 77.5                  & 71.7                   \\
			Shi \etal \cite{ASTER}        &$\surd$            & ResNet                   & MJ+ST        &   Word                  & {93.4}                  & 89.5                     &  94.5 & 91.8                    & 76.1                  & \multicolumn{1}{c}{-} & 78.5                  & 79.5                   \\
			
			Zhan \etal \cite{ESIR}     &$\surd$                & ResNet                   & MJ+ST       &     Word                 & 93.3                  & 90.2                   &  \multicolumn{1}{c}{-}                        & 91.3                     & 76.9                 & - & 79.6                & 83.3                  \\
			
			Baek \etal \cite{wrong} &$\surd$ & ResNet           & MJ+ST        &    Word             & 87.9  &
			87.5                       &{94.9}              &       92.3                & 77.6    & \multicolumn{1}{c}{71.8} & 79.2 &  74.0 \\
			
			Luo \etal \cite{MORAN}   &$\surd$                & ResNet                   & MJ+ST   &  Word      &91.2 &88.3       &    \textbf{95.0}                   & 92.4                           & -               & \multicolumn{1}{c}{68.8} &76.1 & 77.4                \\
			
			Xie \etal \cite{ACE}        &             & ResNet                   & MJ+ST  &   Word      &\multicolumn{1}{c}{-} &\multicolumn{1}{c}{-}      &    \multicolumn{1}{c}{-}                  & \multicolumn{1}{c}{-}                &-&    \multicolumn{1}{c}{68.9}     & 70.1               & 82.6                \\		
			
			
			Wang \etal \cite{DAN}         &            & ResNet                   & MJ+ST    &    Word                     &94.3                 & 89.2                   &  \textbf{95.0}                       & {93.9}              & -                  & \multicolumn{1}{c}{74.5} & 80.0                & 84.4                  \\
			%Song \etal \cite{ReADS}$\star$                     & ResNet                   & MJ+ST  &    Word                     &91.0                 & 91.2            & 96.1                     & 94.5                  & 80.4  & -                & 83.3 & 83.7                   \\
			Luo \etal \cite{Aug}          &           & ResNet                   & MJ+ST  &    Word                     &-                 & -                   &  -                      & -                     & -                  & 76.1  & 79.2                & 84.4                  \\
			Zhang \etal \cite{AutoSTR}          &           & ResNet $\star$                 & MJ+ST &    Word                     &{94.7}                 & \textbf{90.9}                   &  93.3                      & {94.2}                     & {81.8}                  & -  & {81.7}                & -                  \\
			
						
			\hline
			Cheng \etal \cite{FAN}  & & ResNet               & MJ+ST       &    Word+Char          & 87.4                  & 85.9                     & 94.2                     &  93.3                        & 70.6                  &\multicolumn{1}{c}{-} &  \multicolumn{1}{c}{-}                  &   \multicolumn{1}{c|}{-}  \\
			Liao \etal \cite{Perspective}        &             & ResNet                   & MJ+ST    &    Word+Char                     &91.9                 & 86.4                   &  -                       & 91.5                     & -                  & - & -                & 79.9                  \\
			Yang \etal \cite{ScRN}        &$\surd$             & ResNet                   & MJ+ST  &    Word+Char                     &94.4                 & 88.9                   &  95.0                       & 93.9                     & -                  & {78.7} & 80.8                & 87.5                 \\
			Wan \etal \cite{TextScanner}     &                & ResNet                   & MJ+ST  &    Word+Char                     &93.9                 & 90.1            & -                   & 92.9                  & 79.4  & -                & 83.3 & 79.4                   \\
	
			Li \etal \cite{2DATT}        &             & ResNet                   & MJ+ST+P   &  Word      &91.5 &84.5       &    \multicolumn{1}{c}{-}                   &91.0                           & -                & \multicolumn{1}{c}{69.2} & 76.4 & 83.3                \\			
			Yu \etal \cite{SRN}          &           & ResNet                   & MJ+ST+P  &    Word                     & 94.8                 & 91.5                   &  -                 & \textit{95.5}                     & {82.7}                 & -  & {85.1}                & 87.8                  \\
			
			%Wan \etal \cite{TextScanner}                     & ResNet                   & MJ+ST+P  &    Word                     &93.9                 & 90.1            & -                   & 92.9                  & 79.4  & -                & 83.3 & 79.4                   \\
			Hu \etal \cite{GTC}      &               & ResNet                   & MJ+ST+P  &    Word                     & \textit{95.5}                 & \textit{92.9}                   &  \textit{95.2}                  & 94.3                     & 82.5                 & -  & \textit{86.2}                & \textit{92.3}                  \\		
			%{\color{red}TODO new} \etal \cite{ScRN}                     & ResNet                   & MJ+ST         &     Word          &94.3                 & 89.2                   &  95.0                       & 93.9                    & -                  & \multicolumn{1}{c}{74.5} & 80.0               & 84.4                 \\
			
			%\hline
			\hline
			
			%\color{red}{No SPIN}               & VGG                      & MJ                         &   xx                    & xx                         &   xx                      &  xx                        &  xx                     &  xx                     &  xx                      \\
			%SPIN               & VGG                      & MJ                          &  82.3                      &    84.1                      &  91.6                        & 88.7                         &   68.1                    &   \multicolumn{1}{c}{63.4} & 72.3                    &  64.6                      \\
			
			%GA-SPIN                 & VGG                      & MJ                          & 84.1                      & 83.2                         &  92.3                        &   88.7                       & 71.0                      &  \multicolumn{1}{c}{65.1} & 74.5                     &   67.1                     \\
			
			
			%SPIN               & ResNet                      & MJ                          & 83.9                       & 84.6                         &  92.9                        & 88.9                         &   70.6                    &  \multicolumn{1}{c}{65.0} & 75.0                     &  67.4                      \\
			
			%GA-SPIN                 & ResNet                      & MJ                          & 84.2                      & 83.9                         &  93.0                        & 90.0                         &  72.7                     & \multicolumn{1}{c}{67.1} &  76.1                     &  70.1                      \\
			
			%{\color{red}No SPIN}   & ResNet                   &  MJ+ST                          &   xx                    & xx                         &   xx                      &  xx                        &  xx                     &  xx                     &  xx                      \\
			
			SPIN      &$\surd$         & ResNet                   &  MJ+ST         &  Word                  &   {94.7}                    & 87.6                         &   93.4                       &  91.5                        &  79.1                     & \multicolumn{1}{c}{76.0} & 79.7                     &  85.1                      \\
			%GA-SPIN    &$\surd$             & ResNet                   & MJ+ST         &  Word                  &   \underline{94.7}                    & \underline{90.3}                         &  94.4                        & 92.8                         &  \underline{82.2}                     & \underline{78.5} &  \underline{82.8}                    &  \underline{\textbf{87.5}}                      \\
			GA-SPIN    &$\surd$             & ResNet                   & {MJ+ST}         &  Word                  &   \textbf{95.2}                    & \textbf{90.9}                         &  94.9                        & \textbf{94.8}                         &  \textbf{82.8}                     & \textbf{79.5} &  \textbf{83.2}                     &  \textbf{87.5}                      \\
			\hline
		\end{tabular}
	}
	\vspace{-0.1cm}	
	\caption{Comparison with SOTA methods. `P' indicate additionally using extra synthetic or real datasets apart from MJ and ST. `Word' and `Char' in `Supervision' column means word-level and character-level annotations. For IC15, a and b indicate 1811 and 2077 examples, respectively. `Rect' indicates methods focused on rectifications. Method with `$\star$' indicates using multiple backbones for each test set while the others use only one for all test sets. For fair comparison, reported results using additional private data or annotations are not taken into account (Top result in \textit{italic}). Top accuracy for each benchmark is shown in \textbf{bold}. }
%Top accuracy without benchmark validation set is \underline{underlined}.`$\ast$' means using validation set from benchmarks.
	\label{table:3}
	\vspace{-0.3cm}
\end{table*}

\iffalse
\vspace{-0.1cm}
\begin{table*}[!t]
	\centering
	\scalebox{0.75}{
		\begin{tabular}{|l|l|l|l|l|*{8}{p{0.8cm}<{\centering}}|}
			\hline
			\multirow{2}{*}{Methods}  & \multirow{2}{*}{Rect}& \multirow{2}{*}{ConvNet} & \multirow{2}{*}{Training data} & \multirow{2}{*}{Supervision} & \multicolumn{8}{c|}{Benchmark}                                                                                                                                                  \\ \cline{6-12}
			&                          &    &              &              & IIIT                  & SVT                      & IC03                     & IC13                     & IC15a & IC15b                  & SVTP                  & CT                   \\ \hline
			Jaderberg \etal \cite{JaderbergReading}         &      & VGG                      & MJ            &   Word       & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{80.7} & \multicolumn{1}{c}{93.1} & \multicolumn{1}{c}{90.8} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c|}{-} \\
			Shi \etal \cite{CRNN}             &        & VGG                      & MJ          &   Word                   & 78.2                  & 80.8                     & 89.4                     & 86.7                     & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c|}{-} \\
			Shi \etal \cite{RARE}$\star$      &$\surd$              & VGG                      & MJ          &      Word              & 81.9                  & 81.9                     & 90.1                     & 88.6                     & \multicolumn{1}{c}{-} &    \multicolumn{1}{c}{-} & 71.8                  & 59.2                   \\
			Lee \etal  \cite{R2AM}          &        & VGG                      & MJ             &   Word                & 78.4                  & 80.7                     & 88.7                     & 90.0                     & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} &  \multicolumn{1}{c|}{-} \\
			
			
			%Yang \etal \cite{Yang}             & VGG                      & P         &    Word+Char            & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-}    & \multicolumn{1}{c}{-}    & \multicolumn{1}{c}{-}    & \multicolumn{1}{c}{-} &  \multicolumn{1}{c}{-}   & 75.8              & 69.3                   \\
			%Cheng \etal \cite{AON}   & VGG                   & MJ+ST        &    Word            & 87.0        & 82.8                     & 91.5                     &  \multicolumn{1}{c}{-}                     & - &   \multicolumn{1}{c}{68.2} &  73.0         & 76.8 \\			

			
			%Liu \etal \cite{STAR}        &         & ResNet                   & MJ+P      &     Word             & 83.3                  & 83.6                     & 89.9                     & 89.1                     & \multicolumn{1}{c}{-}  & \multicolumn{1}{c}{-} &  73.5                  & \multicolumn{1}{c|}{-} \\
			
			

			
			
			Cheng \etal \cite{FAN}  & & ResNet               & MJ+ST       &    Word+Char          & 87.4                  & 85.9                     & 94.2                     &  93.3                        & 70.6                  &\multicolumn{1}{c}{-} &  \multicolumn{1}{c}{-}                  &   \multicolumn{1}{c|}{-}  \\
			%\hline
			%Shi \etal \cite{CRNN} *                     & VGG                      & MJ+ST                          & 82.9                  & 81.6                     & 93.1                     & 89.2                     & 69.4                  & 70.0                  & 65.5                   \\
			%Shi \etal \cite{RARE} *                    & VGG                      & MJ+ST                          & 86.2                  & 85.8                     & 93.9                     & 91.1                     & 74.5                  & 76.2                  & 70.4                   \\
			%Lee \etal \cite{R2AM} *                 & VGG                      & MJ+ST                          & 83.4                  & 82.4                     & 92.2                     & 88.1                     & 68.9                  & 72.1                  & 64.9                   \\
			%Liu \etal \cite{STAR} *                 & ResNet                   & MJ+ST                          & 87.0                  & 86.9                     & 94.4                     & 91.5                     & 76.1                  & 77.5                  & 71.7                   \\
			Shi \etal \cite{ASTER}$\star$        &$\surd$            & ResNet                   & MJ+ST        &   Word                  & {93.4}                  & 89.5                     &  94.5 & 91.8                    & 76.1                  & \multicolumn{1}{c}{-} & 78.5                  & 79.5                   \\
				
			Zhan \etal \cite{ESIR}$\star$     &$\surd$                & ResNet                   & MJ+ST       &     Word                 & 93.3                  & 90.2                   &  \multicolumn{1}{c}{-}                        & 91.3                     & 76.9                 & - & 79.6                & 83.3                  \\
			
			Baek \etal \cite{wrong}$\star$ &$\surd$ & ResNet           & MJ+ST        &    Word             & 87.9  &
			87.5                       &{94.9}              &       92.3                & 77.6    & \multicolumn{1}{c}{71.8} & 79.2 &  74.0 \\
		
			Li \etal \cite{2DATT}        &             & ResNet                   & MJ+ST+P   &  Word      &91.5 &84.5       &    \multicolumn{1}{c}{-}                   &91.0                           & -                & \multicolumn{1}{c}{69.2} & 76.4 & 83.3                \\
			
			
			Luo \etal \cite{MORAN}$\star$   &$\surd$                & ResNet                   & MJ+ST   &  Word      &91.2 &88.3       &    \textbf{95.0}                   & 92.4                           & -               & \multicolumn{1}{c}{68.8} &76.1 & 77.4                \\
			
			Xie \etal \cite{ACE}        &             & ResNet                   & MJ+ST  &   Word      &\multicolumn{1}{c}{-} &\multicolumn{1}{c}{-}      &    \multicolumn{1}{c}{-}                  & \multicolumn{1}{c}{-}                &-&    \multicolumn{1}{c}{68.9}     & 70.1               & 82.6                \\		
			
			Liao \etal \cite{Perspective}        &             & ResNet                   & MJ+ST    &    Word+Char                     &91.9                 & 86.4                   &  -                       & 91.5                     & -                  & - & -                & 79.9                  \\
			Yang \etal \cite{ScRN}$\star$        &$\surd$             & ResNet                   & MJ+ST  &    Word+Char                     &94.4                 & 88.9                   &  95.0                       & 93.9                     & -                  & \textit{78.7} & 80.8                & 87.5                 \\
			Wang \etal \cite{DAN}         &            & ResNet                   & MJ+ST    &    Word                     &94.3                 & 89.2                   &  \textbf{95.0}                       & \textbf{93.9}                     & -                  & \multicolumn{1}{c}{74.5} & 80.0                & 84.4                  \\
			%Song \etal \cite{ReADS}$\star$                     & ResNet                   & MJ+ST  &    Word                     &91.0                 & 91.2            & 96.1                     & 94.5                  & 80.4  & -                & 83.3 & 83.7                   \\
			Luo \etal \cite{Aug}          &           & ResNet                   & MJ+ST  &    Word                     &-                 & -                   &  -                      & -                     & -                  & 76.1  & 79.2                & 84.4                  \\
			Yu \etal \cite{SRN}          &           & ResNet                   & MJ+ST+P  &    Word                     & 94.8                 & 91.5                   &  -                 & \textit{95.5}                     & \textit{82.7}                 & -  & {85.1}                & 87.8                  \\
			Wan \etal \cite{TextScanner}     &                & ResNet                   & MJ+ST  &    Word+Char                     &93.9                 & 90.1            & -                   & 92.9                  & 79.4  & -                & 83.3 & 79.4                   \\
			%Wan \etal \cite{TextScanner}                     & ResNet                   & MJ+ST+P  &    Word                     &93.9                 & 90.1            & -                   & 92.9                  & 79.4  & -                & 83.3 & 79.4                   \\
			Hu \etal \cite{GTC}      &               & ResNet                   & MJ+ST+P  &    Word                     & \textit{95.5}                 & \textit{92.9}                   &  \textit{95.2}                  & 94.3                     & 82.5                 & -  & \textit{86.2}                & \textit{92.3}                  \\		
			%{\color{red}TODO new} \etal \cite{ScRN}                     & ResNet                   & MJ+ST         &     Word          &94.3                 & 89.2                   &  95.0                       & 93.9                    & -                  & \multicolumn{1}{c}{74.5} & 80.0               & 84.4                 \\
			
			%\hline
			\hline
			
			%\color{red}{No SPIN}               & VGG                      & MJ                         &   xx                    & xx                         &   xx                      &  xx                        &  xx                     &  xx                     &  xx                      \\
			%SPIN               & VGG                      & MJ                          &  82.3                      &    84.1                      &  91.6                        & 88.7                         &   68.1                    &   \multicolumn{1}{c}{63.4} & 72.3                    &  64.6                      \\
			
			%GA-SPIN                 & VGG                      & MJ                          & 84.1                      & 83.2                         &  92.3                        &   88.7                       & 71.0                      &  \multicolumn{1}{c}{65.1} & 74.5                     &   67.1                     \\
			
			
			%SPIN               & ResNet                      & MJ                          & 83.9                       & 84.6                         &  92.9                        & 88.9                         &   70.6                    &  \multicolumn{1}{c}{65.0} & 75.0                     &  67.4                      \\
			
			%GA-SPIN                 & ResNet                      & MJ                          & 84.2                      & 83.9                         &  93.0                        & 90.0                         &  72.7                     & \multicolumn{1}{c}{67.1} &  76.1                     &  70.1                      \\
			
			%{\color{red}No SPIN}   & ResNet                   &  MJ+ST                          &   xx                    & xx                         &   xx                      &  xx                        &  xx                     &  xx                     &  xx                      \\
			
			SPIN$\star$      &$\surd$         & ResNet                   &  MJ+ST         &  Word                  &   \textbf{94.7}                    & 87.6                         &   93.4                       &  91.5                        &  79.1                     & \multicolumn{1}{c}{76.0} & 79.7                     &  85.1                      \\
			GA-SPIN$\star$    &$\surd$             & ResNet                   & MJ+ST         &  Word                  &   \textbf{94.7}                    & \textbf{90.3}                         &  94.4                        & 92.8                         &  \textbf{82.2}                     & \textbf{78.5} &  \textbf{82.8}                     &  \textbf{87.5}                      \\ \hline
		\end{tabular}
	}	
	\caption{Results of SOTA methods. `P' indicate additionally using extra training data apart from MJ and ST. `Word' and `Char' in `Supervision' column means word-level and character-level annotations. Top accuracy for each benchmark is shown in bold. For IC15, a and b indicate 1811 and 2077 examples, respectively. Methods with $\star$ are networks designed for rectifications.}
	\label{table:3}
\end{table*}
\fi
%\vspace{-0.1cm}
\iffalse
\vspace{-0.2cm}
%%supplemental
\subsubsection{{\color{red}Discussion on Regular and Irregular cases.}}
%To explore the importance and effectiveness of the rectification module, we analyze the performance of the proposed module under regular and irregular cases.
The two types of datasets are formerly grouped mainly according to their geometric layout difficulties \cite{wrong}, while it also makes sense in evaluation of our proposed chromatic rectifications as both spatial and color distortions always coexist in relatively complex scenes. In terms of the results of VGG setting for instance from Table \ref{table:2.1}, we find that SPIN w/o AIN has close gain on regular and irregular cases, about +1.0\% on both VGG and ResNet. Then, SPIN can enhance it by largely improving the performance of irregular case (+1.7\%) with few additional parameters. Note it is not surprising \cite{wrong,ASTER,ESIR} can improve the accuracy on irregular datasets more than the regular one because they are intended to rectify texts based on geometric distortions. However, it is inspiring that the spatial-invariance transformation can also achieve similar improvements (approximately +1.0\% under regular case and +1.7\% under irregular case respectively), demonstrating the comparative significance of chromatic rectification. More importantly, obvious enhancement (approximately +1.4\% and +4.3\% under the two cases, respectively) can be observed when equipped with the \textit{GA-SPIN} module, showing the strong ability of integration in geometric and chromatic transformation. The ResNet settings obtain similar conclusions.
\fi
\vspace{-0.2cm}
\subsubsection{Discussion on Different Values of K.}
We empirically analyze the performance under different K values, from 0 to 12, %,  in SPIN and GA-SPIN models.The results are
demonstrated in Fig. \ref{fig:3} with mean accuracy under regular and irregular cases.
%We can conclude from the curves that
{%\color{red}
Both SPIN and GA-SPIN steadily improve the performance when K becomes larger to some extent. %, indicating the effectiveness of chromatic transformations. %A proper value of K=6 is selected.
We do not observe additional performance gain when K is unreasonably large as the smaller K indicates simpler transformation and the larger K may result in complexity and redundancy. While K=3 seems enough for regular text, larger (\eg K=6,9) is better for irregular benchmarks.}
%\vspace{-0.2cm}
\subsubsection{Discussion on Traditional Image Preprocessing.}
%As chromatic difficulties are rarely seen in STR networks, we are the first to extend the rectification stage to a broader perspective of both chromatic and geometric transformation.
As chromatic difficulties are rarely seen in STR networks, we consider traditional image processing techniques for color correction (\eg equalization, binarization, morphological operations).
We try these techniques as preprocessing stage in our recognition task similarly in train and infer phase.
However, they do not work well (even not better than baseline). We attribute it to 2 main reasons:
(1) They suffer from signal loss through image processing operations before flowing into the deep network.
(2) They are manually designed for better image quality according to human intuition and visual feeling, not adapted to variable conditions. %It is indeed the significance of \textit{end-to-end} trainable networks among diverse tasks.	

More details can be found in \textbf{Supplemental Materials}.

%\vspace{-0.3cm}
\vspace{-0.1cm}
%\subsection{Comparison with the State-of-the-Art}
\subsection{Comparison with STN-based Methods}
%Moreover, we observe that MJ dataset simply consists of gray images with plain backgrounds, whereas ST dataset contains color images with complex backgrounds. This could partially explain why the inclusion of the ST dataset significantly enhance the overall performance.
%To further explore the function of chromatic rectification and fusing two kinds of rectifications,
We compare SPIN and GA-SPIN with existing rectification networks in both quantitative and qualitative evaluation. %For fair comparisons, we also report the results under different network architectures, including 7-layer VGG \cite{CRNN} and 32-layer ResNet\cite{FAN}, and under 2 training dataset settings as \cite{wrong}.

\subsubsection{Quantitative Results. }
Table \ref{table:2.1} lists the top results among existing geometric-based transformations \cite{ASTER,ESIR,ScRN} on irregular datasets (more in supplemental materials) with different backbones (VGG-7/ResNet-32) and different training set (MJ/MJ+ST). Both SPIN and GA-SPIN achieve superior recognition performance compared to existing methods. Note the recent ScRN\cite{ScRN} also has impressive performance, but its backbone chooses FPN with ResNet-50 and uses additional explicit supervision with char-level annotations of SynText \cite{ST}.

%The two types of datasets are formerly grouped mainly according to their geometric layout difficulties \cite{wrong}, while it also makes sense in evaluation of our proposed chromatic rectifications as both spatial and color distortions always coexist in relatively complex scenes. In terms of the results of VGG setting for instance from Table \ref{table:2.1}, we find that SPIN w/o AIN has close gain on regular and irregular cases, about +1.0\% on both VGG and ResNet. Then, SPIN can enhance it by largely improving the performance of irregular case (+1.7\%) with few additional parameters. Note it is not surprising \cite{wrong,ASTER,ESIR} can improve the accuracy on irregular datasets more than the regular one because they are intended to rectify texts based on geometric distortions. However, it is inspiring that the spatial-invariance transformation can also achieve similar improvements (approximately +1.0\% under regular case and +1.7\% under irregular case respectively), demonstrating the comparative significance of chromatic rectification. More importantly, obvious enhancement (approximately +1.4\% and +4.3\% under the two cases, respectively) can be observed when equipped with the \textit{GA-SPIN} module, showing the strong ability of integration in geometric and chromatic transformation. The ResNet settings obtain similar conclusions.
\subsubsection{Qualitative Results. }
Some visualization in Fig. \ref{fig:4} clearly shows that the proposed SPIN can rectify the chromatic distortions by adjusting the colors.
The typical chromatic inter-pattern (row 1-3) and intra-pattern (row 4) problems, which the geometric-related rectifications do not consider, can all be mitigated.
%In addition, we can see that GA-SPIN leads to better visual results in both geometric and chromatic perspectives.
Fig. \ref{fig:5} illustrates the rectification effects and text predictions by STN \cite{ASTER}, SPIN and GA-SPIN, respectively. It shows rectifying chromatic distortion can improve the recognition results from two aspects: (1) It makes characters easier to recognize directly. The first 2 rows show that models tend to be misled by special symbols or similar shapes under severe chromatic distortions. At the same time, the proposed SPIN does not over-rectify or degrade images free of chromatic problems, such as the samples in the 3rd row. (2) Chromatic and geometric rectification can promote each other, as clearly shown in the last 2 rows of distorted images with both difficulties. Note in the 4th row, GA-SPIN has superior effects not only in chromatic but also in the geometric perspective over STN-based methods. We attribute it to the chromatic promotion for the geometric transformation.

\vspace{-0.1cm}
%\subsubsection{Evaluation on Overall Performance}
\subsection{Comparison with the State-of-the-Art}
Table \ref{table:3} lists the reported the state-of-the-art results on STR tasks. The proposed SPIN-based rectification network achieves impressive performance across the 7 datasets. % and GA-SPIN ulteriorly boosts the results. %In particular, SPIN consistently outperforms the existing results \cite{CRNN,RARE,MORAN,ESIR, ScRN} under VGG or ResNet backbone trained on the MJ dataset. GA-SPIN further outperforms them by a larger margin.
\subsubsection{Rectification-based Approaches.}
Networks focused on rectification are all denoted in `$\surd$' in Table 4. Although with only word-level annotations, SPIN-based already outperforms all the methods using spatial transformers \cite{ASTER,wrong,ESIR,ScRN} on overall performance(especially in more challenging IC15, SVTP and CT datasets), even when recent method \cite{ScRN} applied heavier backbone and additional char-level annotations.
It points out that despite the widely focused geometric irregularity, color distortions are vital in these complex scenes and SPIN-based methods can effectively boost current performance. %This is why the spatial-invarant module SPIN can obtain comparable performance with the spatial-related ones.
\vspace{-0.1cm}
\subsubsection{Overall Performance among SOTAs.}
Note that even with strong settings like character-level annotations \cite{FAN,Perspective} or deeper convolutional structures (\eg 45-layer ResNet \cite{ASTER,MORAN}) and newly designed advanced framework \cite{DAN}, even compared to reported results using additional real or private data (\eg \cite{TextScanner, ScRN}), SPIN obtains satisfying performance and GA-SPIN shows significant promotion.
Our methods only slightly fall behind (on solely IC03 dataset) the best reported \cite{DAN,MORAN} by 0.1\%, and we attribute the reason to stronger feature extractor (\ie deeper convolution and multi-scale features) and advanced decoupled attention mechanism \cite{DAN}. Advanced networks brings strong ability on regular recognition but fall behind GA-SPIN by a large margin on more complex scenes (\eg IC15, SVTP and CUTE80). In overall performance on 7 benchmarks, our proposed GA-SPIN obviously surpasses all the existing methods under fair comparison. %Note that results with extra supervision or private datasets are not regarded.




==> sections/5_con.tex <==
\vspace{-0.1cm}
\section{Conclusion}
This paper proposes a novel idea of chromatic rectification in scene text recognition. The proposed SPIN allows the channel intensity manipulation of data within the network, giving neural networks the ability to actively transform the input color for clearer patterns.
Extensive experiments show its benefits the performance, especially in more complex scenes.
It is also verified that geometric and chromatic rectifications can be unified into GA-SPIN rather than pipeline of two modules, which further boosts the results and outperform the existing methods by a large margin.
In the future, we are intended to extend it to more general research fields like object classification.%we are intended to extend the chromatic transformer into more general research fields. % like object classification.

